Can Large Language Models Understand Real-World Complex Instructions?

Large language models (LLMs) can understand human instructions, showing their potential for pragmatic applications beyond traditional NLP tasks. However, they still struggle with complex instructions, which can be either complex task descriptions that require multiple tasks and constraints, or complex input that contains long context, noise, heterogeneous information and multi-turn format. Due to these features, LLMs often ignore semantic constraints from task descriptions, generate incorrect formats, violate length or sample count constraints, and be unfaithful to the input text. Existing benchmarks are insufficient to assess LLMs' ability to understand complex instructions, as they are close-ended and simple. To bridge this gap, we propose CELLO, a benchmark for evaluating LLMs' ability to follow complex instructions systematically. We design eight features for complex instructions and construct a comprehensive evaluation dataset from real-world scenarios. We also establish four criteria and develop corresponding metrics, as current ones are inadequate, biased or too strict and coarse-grained. We compare the performance of representative Chinese-oriented and English-oriented models in following complex instructions through extensive experiments. Resources of CELLO are publicly available at https://github.com/Abbey4799/CELLO.

==> 010intro_backup.tex <==
% 真实任务的有什么特色、现有benchmark地不足、MMLU的例子也放到intro



% 大模型的出现revolutionize了自然语言处理领域。它们可以理解人类多样的指令，ranging from casual chatting to complex problem solving. 如何评估大模型的指令遵循能力是重要的研究问题。
The emergence of large language models~(LLMs)~\cite{brown2020language, chowdhery2022palm, touvron2023llama} has revolutionized the field of Natural Language Processing (NLP).
These models are able to understand a wide range of human instructions, spanning from casual conversations~\cite{taori2023stanford} to complex problems solving~\cite{brown2020language}.
Since human instructions are massive and diverse, traditional academic benchmarks that focus on specific tasks are no longer sufficient to evaluate LLMs~\cite{zhong2023agieval, chia2023instructeval}.
% Hence, how to evaluate the instruction-following ability of LLMs is an important research question.

% To this end, 许多针对大模型的benchmark被提出的，它们主要集中在知识、复杂推理、代码层面。它们存在两大问题：一是它们通常只有常见的简单指令。然而，用户在真实场景中的指令是复杂且带有诸多硬性限制的，比如字数限制、输出格式限制、根据材料回答问题的。现有的评估基准无法衡量LLMs对带有硬性约束的复杂指令的理解能力，这导致大模型的实用性存疑。二是The existing benchmarks are generally too challenging for smaller LLMs (below 13 billion parameters), resulting in weak discriminability. For instance, smaller LLMs tend to exhibit an aggregate normalized performance score of 0 on the Big-Bench benchmark~\cite{}. This results in a common scenario where smaller LLMs display comparable deficiencies in reasoning and knowledge~\cite{}. 三是现有的主流评估形式往往为选择题、人工评估、GPT-4自动打分，它们存在评估不稳定、评估主观、结果会受答案长度等bias影响的情况。


% 要聚焦，在complex & fine-grained上，我们指标不是特色，框架才是特色
% (1) 指令太简单 （2）对于有挑战性的任务，评估太严苛、粗糙，导致评分对于小模型没有区分度
Recently, many benchmarks have been proposed to evaluate LLMs from various perspectives such as knowledge~\cite{huang2023c, gu2023xiezhi, yu2023kola}, complex reasoning~\cite{srivastava2023beyond}, and code processing~\cite{chen2021evaluating}.
However, these benchmarks have several limitations.
First, they usually share a few common and simple instructions, while real-world scenarios frequently involve complex instructions~\cite{xu2023wizardlm, luo2023wizardcoder}.
% in terms of their input heterogeneity, length, and noise; output form and content constraints; or multiple task completion requirements.
% 以图~\ref{fig:info}为例，复杂指令pose challenges for existing models, 因为它们在回答时容易忽略对输出形式的要求、统计错误样本数量、忽视任务描述中对内容的约束、对于长输入文本容易产生幻觉。
As shown in Fig.~\ref{fig:010intro}, complex instructions pose challenges to current models.
The models often disregard output format requirements, make sample counting errors, neglect content constraints specified in the task description, and potentially induce hallucinations for lengthy input texts.
% 更异构、更长、更多噪音的输入，对输出的形式、内容有约束，需要同时完成多个任务。
% Consequently, existing benchmarks are inadequate to assess the LLMs’ ability to follow complex instructions with hard constraints, which 
This casts doubt on the practicality of LLMs.
% 对涉及到复杂指令的典型任务（例如tool-using, agent-acting, meta-prompt）上，例如Pass rate的指标太苛刻，导致小模型之间毫无区分度。
Next, when it comes to challenging tasks involving complex instructions, such as tool usage~\cite{qin2023toolllm} and agent action~\cite{liu2023agentbench}, the stringent criteria such as pass rate are too demanding and coarse-grained, resulting in a lack of distinction between smaller models.
Moreover, the mainstream evaluation method for open-ended tasks is GPT-4 automatic scoring, introducing problems such as bias due to varying answer lengths~\cite{wang2023large}.
% 这个地方逻辑有点反了，有一种预设了结论倒推方法的感觉？
% (2) They primarily evaluate abilities that are significantly impacted by the size of the model~\cite{}, resulting in weak discriminability for small LLMs.
% For instance, smaller LLMs tend to exhibit an aggregate normalized performance score of 0 on the Big-Bench benchmark~\cite{}.
% Therefore, a benchmark for complex instruction following, which is more closely related to instruction data quality than model size~\cite{}, can effectively highlight differences in the capabilities of existing smaller LLMs.
% 现有的很多benchmark都是close-ended的，不符合真实应用场景的需求。
% (2) Many existing benchmarks are close-ended, which do not align with the requirements of real-world application scenarios.
% (3) Mainstream evaluation methods for open-ended tasks is GPT-4 automatic scoring, introducing problems such as bias due to varying answer lengths~\cite{}.
% (4) For challenging tasks, the evaluation is too strict and coarse, resulting in low discrimination for small models~\cite{}.

% 攻击评估而不是攻击任务本身

% (2) The existing benchmarks are generally too challenging for smaller LLMs (below 13 billion parameters), resulting in weak discriminability.
% For instance, smaller LLMs tend to exhibit an aggregate normalized performance score of 0 on the Big-Bench benchmark~\cite{}.
% This results in a common scenario where smaller LLMs display comparable deficiencies in reasoning and knowledge~\cite{}.
% (3) Mainstream evaluation methods, such as multiple-choice questions, human evaluation, and GPT-4 automatic scoring, introduce problems such as evaluation instability~\cite{}, subjectivity~\cite{}, and bias due to varying answer lengths~\cite{}.

% 然而，构建一个全面的、实用的、客观的evaluation system for complex instruction with hard constraints following ability is non-trivial, which raises three main concerns: (1) 什么是真实世界场景中人类真正关注的hard constraints? （2）应该选取哪些任务从而提供Holistic view? (3) 如何能客观地评估模型效果，鉴于gpt4打分不准? 
However, establishing a comprehensive, fine-grained, and objective benchmark for complex instruction following is non-trivial, which raises three main concerns:
(1) What criteria should be employed to identify complex instructions?
(2) How to evaluate the model’s complex instructions following ability in a fine-grained way?
(3) How can the model outcomes be objectively assessed?
% （1）如何定义复杂指令？（2）怎么细粒度地评估模型对于复杂指令的理解能力？
% (1) What are the hard constraints that human users care about in real-world scenarios?
% (2) What tasks should be selected to provide a holistic view of the model performance? 
% (3) How can the model outcomes be objectively assessed?





\input{figs/010intro}
\input{figs/030framework}

% In our paper, we establish \texttt{PELICAN}: A Practical Benchmark for Large Language Models' Complex Instructions Following Ability under Hard Constraints. 我们首先从用户的真实需求出发，定义了a set of hard constraints。接着，基于提出的hard constraints，我们搜集并改进了一系列数据，包含x个任务which can be categorized into xx categories. 最终，基于hard constraints，设计了评估系统，以期实现客观的评分。
In this paper, we propose \method, a fine-grained benchmark for evaluating LLMs' complex instruction understanding ability.
The framework of our benchmark is shown in Fig.~\ref{fig:030framework}.
% 首先，我们为复杂指令设计7个评判标准。我们将指令定义为任务描述（必选）和输入文本（可选），并为它们分别设计了评判标准。
% 接着，我们基于评判标准收集了xx条中英双语的复杂指令数据集，包含9类任务。我们提出了两步的数据集构建策略，首先收集数据，并通过纵向和横向两个策略扩充数据集规模和多样性。
% 最后，我们总结了四类约束并设计了对应的自动化指标，以期实现高效的自动化评估。
First, we design seven criteria for complex instructions. 
In our benchmark, instruction is defined as a task description (mandatory) and an input text (optional)~\cite{honovich2022unnatural}.
We devise evaluation criteria based on task description and input text respectively. 
Next, we collect a bilingual (Chinese and English) complex instruction dataset based on our evaluation criteria, containing xxx samples ranging from nine types of tasks.
Specifically, we propose a two-stage dataset construction strategy, which first collects data and then expands the dataset size and diversity through in-depth and in-breadth evolution strategies. 
Finally, we define four types of constraints and design corresponding automated metrics, aiming to achieve efficient automated evaluation.



\hqy{Based our benchmarks, we have the following findings..}

% First, we define a set of hard constraints that capture the authentic demands of users in real-world situations.
% Then, we construct and refine evaluation datasets based on proposed hard constraints, containing xxx samples from xxx tasks, which fall into xxx categories.
% Next, (data evolution...)
% Finally, we design an automatic evaluation system that leverages the hard constraints, aiming to achieve objective and efficient scoring.



% To the best of our knowledge, we are the first to systematically investigate LLMs' complex instructions following ability under hard constraints. To summarize, our contributions are mainly three-fold: (1) 提出了基于硬性约束的大模型复杂指令理解评估系统，总结基于人类实用过程中真正关注的hard constraint并设计了对应的自动评估指标（2）提出了构建基于硬性约束的大模型复杂指令理解数据集的框架，包含数据搜集和数据进化两个环节。我们最终构建了xxx样本，包含xx个任务，可以归为四类。（3）通过大量实验比较了主流模型的复杂指令理解能力
To the best of our knowledge, we are the first to systematically investigate the ability of LLMs to follow complex instructions.
Our contributions are mainly three-fold: 
(1) We propose a comprehensive set of criteria for complex instructions, facilitating both data collection and evaluation criteria design.
(2) We propose a two-stage framework for constructing the evaluation dataset for LLM's complex instruction understanding, including data collection and data evolution.
(3) We construct an evaluation dataset containing xxx samples, covering xx tasks, which fall into xxx categories.
(4) We conduct extensive experiments to compare the complex instruction understanding ability of state-of-the-art models.




% To the best of our knowledge,  we are the first to systematically investigate LLMs' complex instructions following ability under hard constraints.
% To summarize, our contributions are mainly three-fold:
% (1) We propose an evaluation framework that incorporates pertinent hard constraints observed in real-world scenarios, the construction of a dedicated dataset, and the design of an automatic evaluation system.
% (2) We conduct extensive experiments to compare the complex instructions understanding ability of LLMs with different scales.
% (3) We empirically demonstrate that training models with complex instructions under hard constraints can improve their instruction understanding ability.


==> 010intro_backup_v1.tex <==
% The emergence of large language models~(LLMs)~\cite{brown2020language, chowdhery2022palm, touvron2023llama} has revolutionized the field of Natural Language Processing (NLP).
The emergence of large-scale models~\cite{brown2020language, chowdhery2022palm, touvron2023llama} has yielded noteworthy transformations in real-world applications~\cite{richards2023auto, liu2023agentbench}.
These models are able to understand a wide range of human instructions, spanning from casual conversations~\cite{taori2023stanford} to complex problems solving~\cite{brown2020language}.
Since human instructions are massive and diverse, traditional academic benchmarks that focus on specific tasks are no longer sufficient to evaluate LLMs~\cite{zhong2023agieval, chia2023instructeval}.

\input{figs/010intro.tex}
\input{figs/030framework.tex}

% 虽然已经有很多Benchmark从多个角度评估大模型，但没有benchmark关注LLMs对复杂指令的理解，然而复杂指令在真实场景中非常普遍且重要。
% 现有的benchmark不足以有效评估模型的复杂理解能力。
Although many benchmarks have been proposed to evaluate LLMs from various perspectives~\cite{huang2023c, gu2023xiezhi, yu2023kola}, none of them systematically study the complex instructions understanding ability.
Yet, complex instructions are prevalent and crucial in real-world scenarios~\cite{xu2023wizardlm, zhou2023lima}.
% 首先，真实场景的指令往往有形式约束，例如few-shot场景下样本往往需要遵循固定的格式、人类的推理过程可被组织为json形式。形式约束对模型输出的可解析性、可读性都有重要意义。
\textit{First}, real-world instructions often impose constraints on the output format, influencing the parsability and readability of the model's output. 
For instance, samples in few-shot scenarios are usually required to follow a predefined format~\cite{yao2023react}, and the model output imitating human reasoning processes can be structured in JSON format~\cite{liu2023agentbench}. 
% 其次，数量控制也常出现在用户的真实指令中，例如字数限制、句数限制、样本数量控制文章的篇幅。特别地，用户与模型的交互过程是多轮的，例如对字数、样本数量的增删改查，但是现有的benchmark仅包含单轮样本的评估。
\textit{Additionally}, quantity constraints are common during instruction understanding, such as restrictions on word count, sentence count, or sample count to regulate the length of model output~\cite{zhou2023controlled, yao2023collie}.
% 接着，用户真实的任务描述中往往带有对语义的细粒度限制。例如，要求回答包含key elements、限制回答的标签范围、预定义可调用的函数。
\textit{Also}, users often specify detailed semantic restrictions in task descriptions, such as the inclusion of key elements~\cite{zhou2023lima} or the use of predefined callable functions~\cite{liu2023agentbench}.
\textit{Moreover}, in real-life scenarios, the input text often comprises lengthy, noisy, and heterogeneous information, thereby posing challenges for LLMs to locate and be faithful to the relevant information in the given document~\cite{li2023halueval, an2023eval}.
\textit{Furthermore}, the interaction process between users and models is multi-turn~\cite{zhou2023lima}, involving consistent modifications such as adding, deleting, or modifying content.
% However, the existing benchmarks solely encompass the evaluation of single-turn samples.
Overall, real-world instructions involve the composition of multiple features (Fig.\ref{fig:010intro}).

% 虽然已有Benchmark涉及到部分上述和复杂指令相关的特征，例如count restriction, semantic restriction, long text understanding，但是一方面，它们的指令普遍比较简单，不符合真实的应用场景，另一方面，它们往往只涉及了单一的特征，而真实场景往往是组合了多个特征。
Existing benchmarks are insufficient for effectively assessing the ability of LLMs to understand complex instructions for the following reasons.
First, as shown in Fig.~\ref{fig:010intro}, existing benchmarks are either close-ended~\cite{huang2023c, zhong2023agieval} or contain common and simple instructions~\cite{yu2023kola, srivastava2023beyond}, which fail to mirror the complexity of real-world instructions.
Additionally, though certain benchmarks cover some of the above features of complex instructions, such as count restriction~\cite{zhou2023controlled, yao2023collie}, semantic restriction~\cite{chen2022controllable}, and long text understanding~\cite{an2023eval}, they only encompass isolated features, while real-world instructions involve the composition of these features~(Fig.\ref{fig:010intro}).
% 虽然已有Benchmark包含组合了上述多个复杂特征的指令，但是它们的评估聚焦于模型是否能自主完成任务。他们采用的非黑即白的pass rate评估指标评估标准太严格、粗粒度，导致小模型普遍得分几乎为0，没有区分度。
Moreover, although some benchmarks incorporate instructions combining multiple complex features~\cite{qin2023toolllm, liu2023agentbench}, the evaluation criteria employed have several limitations.
% they focus on whether models can automatically complete the goal.
% However, 
On one hand, the binary pass rate is strict and coarse-grained, resulting in universally low scores for smaller LLM without discrimination~\cite{liu2023agentbench}.
On the other hand, GPT-4 automatic scoring introduces problems such as bias due to varying answer lengths~\cite{wang2023large}.
% However, the evaluation criteria employed, namely the binary pass rate, is strict and coarse-grained, resulting in universally low scores for smaller LLM without discrimination.
% 复杂指令，但它们的评估标准太coarse-grained，导致对小模型没有区分度。
% 总而言之，已有的benchmarks及其对应的指标不足以全面且细粒度地反应模型对真实场景中复杂指令的理解能力。
Consequently, the existing benchmarks and their corresponding metrics are insufficient to comprehensively and granularly reflect the ability of LLMs to understand complex instructions in real scenarios.


However, establishing a comprehensive and fine-grained benchmark for complex instruction following is non-trivial, which raises three main concerns:
(1) What features should be considered to identify complex instructions comprehensively?
(2) How to construct complex instruction datasets that faithfully mirror real-world scenarios?
(3) How to assess the ability of LLMs to follow complex instructions at a fine-grained level, in order to attain discriminative results?


In this paper, we propose \method, a fine-grained benchmark to evaluate the \textbf{\underline{C}}ompl\textbf{\underline{E}}x instruction understanding ability of \textbf{\underline{L}}arge \textbf{\underline{L}}anguage M\textbf{\underline{O}}dels.
The framework of our benchmark is shown in Fig.~\ref{fig:030framework}.
% 首先，我们为复杂指令设计7个评判标准。我们将指令定义为任务描述（必选）和输入文本（可选），并为它们分别设计了评判标准。
% 接着，我们基于评判标准收集了xx条中英双语的复杂指令数据集，包含9类任务。我们提出了两步的数据集构建策略，首先收集数据，并通过纵向和横向两个策略扩充数据集规模和多样性。
% 最后，我们总结了四类约束并设计了对应的自动化指标，以期实现高效的自动化评估。
% 对于现有的benchmarks仅覆盖Isolated features of complex instruction的问题，我们首先设计了8个criteria for complex instructions并提出了一个两阶段的framework去构建复杂指令评估数据集。
As existing benchmarks only cover isolated features of complex instructions, we first design eight features for complex instructions, then propose a two-stage framework to construct an evaluation dataset that reflects real-world situations by encompassing a composition of our devised features.
% 对于现有包含多个feature的复杂指令数据集评估标准太严格单一的问题，我们定义了四类限制并设计了对应的自动化评估标准。
Since the evaluation criteria for existing complex instruction datasets are too stringent and coarse-grained, we define four types of criteria and design corresponding automated evaluation metrics.
% 我们通过大量的实验证明，我们提出的评估指标可以更细粒度、更有区分度地对比现有的模型。
We conduct extensive experiments to prove that our evaluation metrics can granularly and distinctly compare existing models.
Overall, our contributions are mainly four-fold: 
\begin{itemize}
    \item To the best of our knowledge, we are the first to systematically investigate the ability of LLMs to follow complex instructions. 
We propose a comprehensive set of features for complex instructions, facilitating both dataset construction and evaluation criteria design.
    \item We propose a two-stage framework for constructing the evaluation dataset for LLM's complex instruction understanding, including data collection and data evolution. 
We finally construct a Chinese complex instruction dataset based on our evaluation criteria, containing \num samples covering nine tasks.
    \item We design four evaluation criteria and corresponding automatic metrics, which are empirically demonstrated to assess LLMs' ability to understand complex instructions in a more fine-grained and discriminative way.
    % 分析了不同主导语言的模型对中文复杂指令的理解能力
    \item We compare 19 representative Chinese-oriented models and 14 representative English-oriented models' performance on our benchmark.
\end{itemize}

% First, we design seven criteria for complex instructions. 
% In our benchmark, instruction is defined as a task description (mandatory) and an input text (optional)~\cite{honovich2022unnatural}.
% We devise evaluation criteria based on task description and input text respectively. 
% Next, we collect a bilingual (Chinese and English) complex instruction dataset based on our evaluation criteria, containing xxx samples ranging from nine types of tasks.
% Specifically, we propose a two-stage dataset construction strategy, which first collects data and then expands the dataset size and diversity through in-depth and in-breadth evolution strategies. 
% Finally, we define four types of constraints and design corresponding automated metrics, aiming to achieve efficient automated evaluation.


% 如何构建真实场景中的复杂指令数据集，让它们是复杂指令的评估标准的组合？
% (2) How to evaluate the model’s complex instructions following ability in a fine-grained way?

% 如何细粒度地评估模型理解复杂指令的能力，让结果有一定区分度？
% (3) How can the model outcomes be objectively assessed?

% In this paper，我们提出xxx。为了搜集更复杂的数据，我们criteria + construct data。为了让小模型更有区分度，我们xxx。



% Our main contributions



==> 010intro_backup_v2.tex <==
The emergence of large-scale models~\cite{brown2020language, chowdhery2022palm, touvron2023llama} has yielded noteworthy transformations in real-world applications~\cite{richards2023auto, liu2023agentbench}.
These models are able to understand a wide range of human instructions, spanning from casual conversations~\cite{taori2023stanford} to complex problems solving~\cite{brown2020language}.
Since human instructions are massive and diverse, traditional academic benchmarks that focus on specific tasks are no longer sufficient to evaluate LLMs~\cite{zhong2023agieval, chia2023instructeval}.

\input{figs/010intro.tex}
\input{figs/030framework.tex}

% 复杂指令的理解对模型而言是个有挑战的事



In general, complex instructions understanding remains quite challenging for LLMs~\cite{xu2023wizardlm, luo2023wizardcoder, zhou2023lima}.
% 什么是复杂指令？为什么有挑战？
Instruction generally consists of two parts~\cite{honovich2022unnatural}: \textit{Task description} (mandatory) describes the task goal and \textit{Input text} (optional) provides reference texts for the model to answer questions or the history of multi-turn conversations, as shown in Fig.~\ref{fig:010intro}.

% real-world instruction有很多复杂指令，而不是传统的Benchmark中的简单的指令，可以稍微展开。
% 还是想把task description点出来，我怕审稿人觉得complex task是指BBH那种complex reasoning
Hence, there can be two categories of complex instructions: \textit{complex task descriptions} and \textit{complex input}.
Regarding \textit{complex task descriptions}, models need to undertake multiple tasks (i.e. \underline{multi-tasking)} and there can be diverse restrictions describing the task, including \underline{semantics constraints} (e.g. the inclusion of key elements~\cite{zhou2023lima} or the use of predefined callable functions~\cite{liu2023agentbench}), \underline{format constraints} (e.g. the predefined format in few-shot scenarios~\cite{yao2023react} or structured format imitating human reasoning processes~\cite{liu2023agentbench}), \underline{quantity constraints} (e.g. word, sentence, or sample count regulating the length of model output~\cite{zhou2023controlled, yao2023collie}).
Regarding \textit{complex input}, the input text generally have \underline{long context}~\cite{an2023eval, liu2023lost}, \underline{noise} (e.g. colloquial expressions~\cite{guo2023close} and error accumulation caused by pipeline method~\cite{sun2023chatgpt}), \underline{heterogeneous information} (e.g. a combination of structured and unstructured data~\cite{zha2023tablegpt}), and in the form of \underline{multi-turn}~\cite{ding2023enhancing}.

% 现实应用指令的复杂性attribute to account for many existing errors of LLMs, posing challenges for LLMs
Owing to the above features of complex instructions also depicted in Fig.~\ref{fig:030framework}, LLMs often encounter \textit{four} types of errors during complex instruction understanding.
As shown in Fig.~\ref{fig:010intro}, LLMs may (1) ignore \underline{semantic constraints} from task description(s)~\cite{zhou2023lima}, (2) generate answers in incorrect \underline{format}~\cite{qin2023toolllm}, or (3) violate the length or sample \underline{count constraints}~\cite{zhou2023controlled}, especially when \underline{multiple tasks} are required to be performed.
Moreover, models can (4) be unfaithful to the input text, especially when it is \underline{long}, \underline{noisy}, \underline{heterogeneous} or in the form of \underline{multi-turn}~\cite{li2023halueval, an2023eval}.
Overall, complex instruction following pose challenges to current models.

However, existing benchmarks are insufficient for effectively assessing the ability of LLMs to understand complex instructions.
On one hand, Fig.~\ref{fig:010intro} shows that existing benchmarks are either close-ended~\cite{huang2023c, zhong2023agieval, yu2023kola, hendrycks2020measuring} or contain common and simple instructions~\cite{srivastava2023beyond, chia2023instructeval, dubois2023alpacafarm}, which fail to mirror the complexity of real-world instructions.
On the other hand, even though certain benchmarks cover some of the above features of complex instructions, such as count restriction~\cite{zhou2023controlled, yao2023collie}, semantic restriction~\cite{chen2022controllable}, and long text understanding~\cite{an2023eval}, they only encompass isolated features, while real-world instructions comprehensively cover these features~\cite{zhou2023lima}.
Overall, none of existing benchmarks systematically study the complex instructions understanding ability of LLMs.

In this paper, we propose \method, a benchmark for evaluating LLMs' ability to follow complex instructions systematically.
The framework of our benchmark is shown in Fig.~\ref{fig:030framework}.


% 稍微解释一下close-ended，去掉那么多citation
% 我们从八个维度刻画复杂指令，建framework to复杂指令的框架with eight features
% Accordingly, we propose a novel evaluation system. 再说为什么现有的benchmark不足
% citation 空格 binary pass rate，strict and coarse-grained太vague了
% propose criteria
As existing benchmarks only cover isolated features of complex instructions, we first design eight features for complex instructions and construct an evaluation dataset covering these features comprehensively.
The current evaluation criteria are insufficient to comprehensively reflect the ability of LLMs to understand complex instructions for the following reasons.
First, complex instructions in real-world scenarios are open-ended~\cite{xu2023wizardlm}, thus the criteria commonly used for close-ended benchmarks are not suitable in such cases~\cite{hendrycks2020measuring}.
Moreover, many studies adopt GPT4 evaluation for automated open-ended assessment, which introduces bias problems\cite{wang2023large}.
Furthermore, the binary pass rate adopted by the benchmarks containing complex instructions is strict and coarse-grained, resulting in universally low scores for smaller LLM without discrimination~\cite{liu2023agentbench, qin2023toolllm}.
Hence, we establish four criteria based on the four types of errors that LLMs might face while comprehending instruction, as previously introduced, and develop corresponding metrics to evaluate them automatically.
Overall, our contributions are mainly four-fold: 
\begin{itemize}
    \item To the best of our knowledge, we are the first to systematically investigate the ability of LLMs to follow complex instructions. 
We propose a comprehensive set of features for complex instructions, facilitating both dataset construction and evaluation criteria design.
    \item We construct a complex instruction dataset from real-world scenarios, containing \num samples encompassing nine tasks, effectively covering our specified features.
    Specifically, we propose a two-stage framework for constructing the evaluation dataset for LLM's complex instruction understanding.
    \item We design four evaluation criteria and corresponding automatic metrics for assessing LLMs' ability to understand complex instructions in a comprehensive and discriminative way.
    % 分析了不同主导语言的模型对中文复杂指令的理解能力
    \item We compare \modelNumch representative Chinese-oriented models and \modelNumeg representative English-oriented models' performance on our benchmark.
\end{itemize}


==> tables/030examples.tex <==
\begin{figure}[t] 
    \centering
        \includegraphics[width=1.0\linewidth]{temp_figs/examples.png} 
    \captionsetup{font={small}} 
    \label{fig:intro}
\end{figure}

==> tables/030labeling.tex <==
\begin{figure}[t] 
    \centering
        \includegraphics[width=1.0\linewidth]{temp_figs/labeling.png} 
    \captionsetup{font={small}} 
    \label{fig:intro}
\end{figure}
